Make-A-Character 2: Animatable 3D Character Generation From a Single Image

This report introduces Make-A-Character 2, an advanced system for generating high-quality 3D characters from single portrait photographs, ideal for game development and digital human applications. Make-A-Character 2 builds upon its predecessor by incorporating several significant improvements for image-based head generation. We utilize the IC-Light method to correct non-ideal illumination in input photos and apply neural network-based color correction to harmonize skin tones between the photos and game engine renders. We also employ the Hierarchical Representation Network to capture high-frequency facial structures and conduct adaptive skeleton calibration for accurate and expressive facial animations. The entire image-to-3D-character generation process takes less than 2 minutes. Furthermore, we leverage transformer architecture to generate co-speech facial and gesture actions, enabling real-time conversation with the generated character. These technologies have been integrated into our conversational AI avatar products.

==> 10_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}



==> 13_results.tex <==
\section{Results}
\label{sec:Results}







==> 14_future.tex <==
\section{Future Work}
\label{sec:Future}
Our current version focuses on generating visually appealing 3D avatars of Asian ethnicity, as our selected SD model is primarily trained on Asian facial images. In the future, we will try to expand support for different ethnicities and styles.
It is worth noting that our de-lighting datasets consist of clean face textures only, non-natural facial patterns like scribbles or stickers may be weakened in the generated avatars. Currently, our garments and body parts are pre-produced and matched based on textual similarity. However, we are actively working on developing cloth, expression, and motion generation techniques driven by text prompts.





==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

